Automated CFI Policy Assessment with Reckon

Protecting programs against control-flow hijacking attacks recently has become an arms race between defenders and attackers. While certain defenses, e.g., \textit{Control Flow Integrity} (CFI), restrict the targets of indirect control-flow transfers through static and dynamic analysis, attackers could search the program for available gadgets that fall into the legitimate target sets to bypass the defenses. There are several tools helping both attackers in developing exploits and analysts in strengthening their defenses. Yet, these tools fail to adequately (1) model the deployed defenses, (2) compare them in a head-to-head way, and (3) use program semantic information to help craft the attack and the countermeasures. Control Flow Integrity (CFI) has proved to be one of the promising defenses against control flow hijacks and tons of efforts have been made to improve CFI in various ways in the past decade. However, there is a lack of a systematic assessment of the existing CFI defenses. In this paper, we present Reckon, a static source code analysis tool for assessing state-of-the-art static CFI defenses, by first precisely modeling them and then evaluating them in a unified framework. Reckon helps determine the level of security offered by different CFI defenses, and find usable code gadgets even after the CFI defenses were applied, thus providing an important step towards successful exploits and stronger defenses. We have used Reckon to assess eight state-of-the-art static CFI defenses on real-world programs such as Google's Chrome and Apache Httpd. Reckon provides precise measurements of the residual attack surfaces, and accordingly ranks CFI policies against each other. It also successfully paves the way to construct code reuse attacks and to eliminate the remaining attack surface, by disclosing calltargets under one of the most restrictive CFI defenses.

==> parts/abstract.tex <==
%Long version:
% Code reuse attacks (CRAs) are used to hijack the control
% flow of a program in order to execute malicious activities on a
% host computer under partial stealth protection.
% In order to reason about the level of protection of the plethora of tools
% used against illegal indirect control flow transfer based attacks
% there is the need for metric(s) which can asses precisely qualitatively and quantitatively
% the protection level after a mitigation technique was enforced.
% Current solutions such as the AIR, fAIR and AIA metrics can measure
% indirect transfers without any particular focus on any CRAs attack. 
% These metrics are mostly crafted in such a way that the results w.r.t. the level 
% of protection is mostly above 90\%.
% We argue that since these metrics are only capable to compute average
% values without the possibility to reason about single (il)legal indirect
% control flow program transfers these are mostly useless.
% 
% In this paper, we propose a novel CRAs formalization framework (ICFI) 
% which can help to better asses code reuse attacks:
% \textit{1)} surface reduction,
% \textit{2)} runtime protection damping, and
% \textit{3)} gadgets availability after a CFI-based policy was applied.
% Based on ICFI we propose a systematic approach used to formalize six
% precise metrics for reasoning about CRAs that are based on
% forward-edges and backward-edges in program binaries and C/C++ source code.
% These six novel metrics can be used to precisely reason about
% the above stated limitations.
% We evaluate our six metrics by putting them to work in a case study in which we identify
% optimal protection levels for Chrome, Firefox and the Spec CPU2006 benchmark.
% We correlate our analysis results with the security level of 5
% state-of-the-art binary and 5 state-of-the-art source code CFI-based protection tools, 
% respectively. Finally, we give other optimal choices which are more aggressively tuned
% % with a higher (or lower) runtime penalty but with an optimal reduced attack surface.
% 
% 
% %Short Version:
% Code reuse attacks (CRAs) are used to hijack the control
% flow of a program in order to perform malicious turing complete computations.
% Current solutions for assessing the attack surface after a control flow integrity (CFI) policy was applied can measure
% only indirect transfer averages in best case without providing any insights w.r.t. the absolute calltarget reduction per
% callsite, runtime overhead and gadget availability. Further, tool comparison 
% is poor or not possible at all.
% 
% In this paper, we propose a novel CRAs reasoning framework (ICFI) 
% which can help to consistently asses CRAs w.r.t.:
% (1) attack surface reduction,
% (2) runtime performance overhead damping, and
% (3) gadgets availability after a CFI-based policy was enforced.
% Based on ICFI we propose a systematic approach used to formalize six
% precise metrics for reasoning about CRAs mitigation techniques that are based on
% forward-edges and backward-edges in binaries and source code of C++ programs.
% We evaluated ICFI by putting it to work in a case study in which we
% assessed the protection level of several CFI-based policy enforcement tools.
% We were able for the first time to consistently compare these tools against each other.
% 
% Finally, we hope that our ICFI reasoning framework will be used in future by other researchers
% to asses new CFI-based tools and to aid the comparison between these tools by using
% a consistent reasoning framework.
%
% Mat: too verbose, cut down to make the abstract crisper.
%
% Ever since the first Return Oriented Programming (ROP) attack was presented the cat and mouse game between defenders and attackers
% has seen several peaks on both sides w.r.t. to the fact that defenses got more effective while the attacks got more advanced over time.
% As in principle performing exploits in the face of this myriad of defenses it is still possible, in
% practice the situation is different. The attacker is confronted with the situation that he has to search in the protected program or in the source code
% of the protected program for gadgets which he can still use for his exploit after a defense was deployed.
% On one hand, most static gadget discovery tools are performing 
% primitive static searches on the binary of the protected program in order to find useful
% gadgets. On the other hand, the dynamic analysis tools perform dynamic analysis of the protected program in order to find usable gadgets.
% Interestingly to note is that, as the bar for the attacker is continuously raised by each new defense, these tools assisting the attacker when 
% searching for gadgets still lack to:
% (1) model the deployed defense, and
% (2) use semantic program information in order to be able help craft an attack.
%%% Rewrite of the above but shorter and more to the point:

Protecting programs against control-flow hijacking attacks recently has become an arms race between defenders and attackers. While certain defenses, e.g., \textit{Control Flow Integrity} (CFI), restrict the
targets of indirect control-flow transfers through static and dynamic analysis,
attackers could search the program for available gadgets that fall into the legitimate target sets
to bypass the defenses.
% attackers explore these target sets and leverage control over data, exposing
% weaknesses in the defenses.
% %
% %An attacker searches the program to find available code reuse attack gadgets in order to construct viable exploits.
% %jasper:
% In order to construct viable exploits, attackers search the program for available gadgets.
%
%Several tools that can help attackers develop exploits as well as analysts to strengthen defenses currently exist. 
%jasper
There are several tools helping both attackers in developing exploits and analysts in strengthening their defenses.
Yet, these tools fail to adequately
(1) model the deployed defenses, 
(2) compare them in a head-to-head way, and 
(3) use program semantic information to help craft the attack and the countermeasures.

Control Flow Integrity (CFI) has proved to be one of the promising defenses against control flow hijacks and tons of efforts have been made to improve CFI in various ways in the past decade. However, there is a lack of a systematic assessment of the existing CFI defenses. In this paper, we present \sysname, a static source code analysis tool for assessing state-of-the-art static CFI defenses, by first precisely modeling them and then evaluating them in a unified framework. \sysname helps determine the level of security offered by different CFI defenses, and find usable code gadgets even after the CFI defenses were applied, thus providing an important step towards successful exploits and stronger defenses. We have used \sysname to assess eight state-of-the-art static CFI defenses on real-world programs such as Google's Chrome and Apache Httpd.
% We provide precise measurements of the remaining attack surface and we were for the first time able to rank the CFI defenses.
% \paul{I did add the previous sentence. Is it ok? should I add some concrete numbers?}
% \chao{we need data to argue how good \sysname is.}
\sysname provides precise measurements of the residual attack surfaces, and accordingly ranks CFI policies against each other. It also successfully paves the way to construct code reuse attacks and to eliminate the remaining attack surface, by disclosing calltargets under one of the most restrictive CFI defenses.
% \paul{I have added by disclosing calltargets ...}
% \chao{how does \sysname help defense?}
% We demonstrate, based on a NodeJS case study, the usefulness of \sysname when crafting code reuse attacks with a state-of-the-art CFI code reuse defense in place.
% Finally, we present yet another highly relevant application of \sysname, in which it can be used to 
% perform precise CFI relevant measurements in conjunction with novel CFI metrics.
% \mat{Mention actual results, not just that we're great.}
% \mat{Remove comments if you think you have addressed them. That's what git
% revision history is for.}


==> parts/application.tex <==
Here we present how \sysname 
performs different types of CFI-related measurements.
\sysname helps to provide precise and reproducible measurement 
results when performing CFI-related investigations. This section provides several alternatives to existing limited
CFI metrics: AIR~\cite{mingwei:sekar}, fAIR~\cite{vtv:tice}, and AIA~\cite{aia}, which provide average result values w.r.t. only forward 
edges calltarget set reduction per callsite after a certain CFI policy was applied 
to a program. Further, we will show with which novel CFI-related policies 
\sysname can be used in conjunction. Another set of metrics was
introduced in a recent survey by Burow \textit{et al.}~\cite{cfi:survey};
we evaluate our metrics on real-world programs while in the survey the authors
evaluate their metrics on a per-mechanism basis, changing the point of view.
Finally, for space reasons we focus on the most widely used ones.
\vspace{-.2cm}
\begin{figure}[ht]
\captionsetup{justification=justified}
\centering
\tikz \node [scale=.67, inner sep=0] {
 \begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum width=2em]
  {
%       \textbf{CSD}  &                & \textbf{bCGA}     &\textbf{RSD}         \\
                    &                & \textbf{bCGA}     &                    \\
      \textbf{CTR}  & ics            & irs               &\textbf{RTR}        \\
      VT            & CH             & CFG               &P                   \\
      VTH           & \textbf{fCGA}  & CG                &                    \\};
  \path[-stealth]
    (m-2-2) edge node [above] {$inside$} (m-3-2) %ICS - CH
    (m-2-1) edge [dashed] node [above] {$uses$} (m-2-2) %iCTR - ICS
    (m-2-1) edge [dashed] node [left] {$uses$} (m-3-2) %iCTR - CH
    (m-3-3) edge node [below] {$abstraction$} (m-3-4) %CFG - P
    (m-3-1) edge node [above] {$subpart$} (m-4-1) %VT- VTH
    (m-4-1) edge node [below] {$subpart$} (m-3-2) %VTH - CH
    (m-3-1.east|-m-3-2) edge node [below] {$subpart$} (m-3-2) %VT- CH
    (m-3-2.east|-m-3-3) edge node [below] {$abstraction$} (m-3-3) %CH- CFG
    (m-4-3) edge node [below] {$contained$} (m-3-3) %CG - CFG
%     (m-1-1) edge [dashed] node [above] {$uses$} (m-2-1) %CSD - iCTR
    
    (m-4-2) edge [dashed] node [above] {$uses$} (m-3-2) %fCGA - CH
    (m-4-3) edge [dashed] node [above] {$uses$} (m-4-2) %CG - fCGA
    
%     (m-1-4) edge [dashed] node [above] {$uses$} (m-2-4) %RSD - iRTR
    (m-2-4) edge [dashed] node [above] {$uses$} (m-2-3) %iRTR - IR
    (m-2-3) edge [dashed] node [below] {$uses$} (m-3-2) %IRS - CH
    
    (m-2-3) edge [dashed] node [above] {$coupled$} (m-2-2) %IRS - ICS
    (m-1-3) edge [dashed] node [above] {$depends$} (m-2-2) %bCGA - ICS
    (m-1-3) edge [dashed] node [above] {$uses$} (m-2-3) %bCGA - IRS
    
    (m-2-4) edge [dashed] node [below] {$uses$} (m-3-2) %iRTR - CH
    ;
\end{tikzpicture}};
% \centering
\caption{Relationships between our four metrics (bold text), and
program metadata primitives.}
\label{Interaction of forward-edge related concepts.}
\end{figure}

Figure~\ref{Interaction of forward-edge related concepts.} depicts the relationships between our 
metrics and program primitives. In 
Figure~\ref{Interaction of forward-edge related concepts.},
we use the following abbreviations:
% \begin{enumerate}[labelindent=0pt]
%  \item 
(1) \emph{ics:} indirect call site (\textit{i.e.,} x86 \texttt{call} instruction);
%  \item 
(2) \emph{irs:} indirect return site (\textit{i.e.,} x86 \texttt{ret} instruction);
%  \item 
(3) \emph{P:} program;
%  \itedm 
(4) \emph{VT:} virtual table;
%  \item 
(5) \emph{VTI:} virtual table inheritance;
%  \item 
(6) \emph{CH:} class hierarchy;
%  \item 
(7) \emph{CFG:} control flow graph;
%  \item 
(8) \emph{CG:} code reuse gadget;
%  \item 
Metrics: (9) \emph{CTR:} indirect call target reduction;
%  \item 
% (10) \emph{CSD:} indirect call site damping metric;
%  \item 
(10) \emph{RTR:} indirect return target reduction;
%  \item 
% (12) \emph{RSD:} indirect return site damping metric;
%  \item 
(11) \emph{fCGA:} forward-edge based $CG$ availability;
%  \item 
(12) \emph{bCGA:} backward return-edge based $CG$ availability.
% \end{enumerate}

Based on the two observations: (1) \sysname allows to determine precise forward edge mappings as
well as backward edge mappings when the forward edge mapping is available due to the caller callee function
calling convention, and (2) \sysname can be used to search for the presence of code reuse gadgets 
(\textit{i.e.,} COOP gadgets which are complete virtual functions).

Next, we formulate four advantages of our approach:
(1) our metrics do not provide average numbers but rather absolute values,
(2) can be used to assess backward edge target set reduction,
(3) can be used to assess the forward and backward edge control flow transfer damping due to a variable number of checks inserted before each indirect control flow transfer, and
(4) can be used to assess the forward and backward edge control flow transfers w.r.t. gadget availability. 
Finally, we present our four CFI metrics which can be used in conjunction with \sysname.

\newcommand{\ctr}{\mathit{ctr}}

\begin{definition}[\textbf{CTR}]
Let $ics_{i}$ be a particular indirect callsite in a program $P$,
$\ctr_{i}$ is the total number of legitimate calltargets for an $ics_{i}$ 
after hardening a program with a certain CFI policy.
\label{ctr label}
\end{definition}
Then the $iCTR$ metric is:
% \begin{equation}
$CTR = \sum_{i=1}^n \ctr_{i}$.
% \end{equation}
Note that the lower the value of $CTR$ is for a given program, the more precise the CFI policy 
is. The optimal value of this metric is equal to the total number of callsites present 
in the hardened program. This means that there is a one-to-one mapping.
We can also capture the distribution of the numbers of call targets
using min, max, and standard deviation functions.
% \mat{@Mathias P. can you please do this one: Discuss false positives where a CFI policy may underapproximate (i.e., less
% than the allowed targets for a site); this could lead to imprecision as the sum
% assumes that you always add the full set of allowed targets for each call site.
% Dynamic policies may under-approximate and only allow targets on demand.}
% 
% Paul: I fully agree, but the under-approximation issue is related to only dynamic CFI policies but 
% our policies are static CFI policies, see Table 1. for clarifications.
% 
% \mat{The problem is that your metric fails if a CFI policy is under-approximate.
% Think about piCFI which only activates on a per-input basis (or PittyPat). Your
% metric does not work for policies that change the sets at runtime. 
% Paul: right I agree, but our CFI policies are static. We exclude runtime based CFI policies. See Table 1.
% You need to
% address this. There are different options to address it, so I can't really pick
% one for you.}
% Mat: Reviewers may ask this question, so you need to clarify. I'm trying to
% highlight pitfalls that a reviewer/reader may see. An author's goal is to
% reduce/remove as many pitfalls as possible. Make it easy for the reader to
% understand your paper!
%
% \begin{itemize}
% \item 
Minimum: $\min_{i}{\{\ctr_{i}\}}$;
Maximum: $\max_{i}{\{\ctr_{i}\}}$; and
Standard Deviation (SD): $CTR_{SD} = \sqrt{\frac{\sum_{i=1}^n ({ctr_{i} - \overline{ctr_{i}}})^2}{n}}\label{ctrsd}$.

\begin{definition}[\textbf{RTR}]
Let $irs_{i}$ be a particular indirect return site in the program $P$,
$rtr_{i}$ is the total number of available return targets for each $irs_{i}$ 
after hardening the backward edge of a program with a CFI policy.
\label{rtr definition.}
\end{definition}
Then the $RTR$ metric is:
% \begin{equation}
$RTR = \sum_{i=1}^n rtr_{i}$.
% \end{equation}
Note that as lower the value of $RTR$ is for a given program, the better the CFI policy 
is. The optimal value of this metric is equal to the total number of indirect return sites present 
in the hardened program. This means that there is a one-to-one mapping.
Other key properties:
% \begin{itemize}
Minimum: $RTR_{MIN} = \min_{i}{\{rtr_i\}}$;
Maximum: $RTR_{MAX} = \max_{i}{\{rtr_i\}}$; and
Standard Deviation (SD): $RTR_{SD} = \sqrt{\frac{\sum_{i=1}^n {(rtr_{i} - \overline{rtr_{i}})}^2}{n}}$.

%%put afterwards in appendix
% \begin{definition}[\textbf{CSD}]
%  Let $ncn_{i}$ be the runtime cost for a CFI check located before an indirect callsite $ics_{i}$ which
%  is present in a given hardened program. 
%   Let $k$ be the runtime overhead (damping ratio) imposed by one inserted CFI check at the $irs_{i}$.
%   The $k$ value could represent milliseconds needed to perform a CFI check.
% \label{csd definition.}
% \end{definition}
% Then the $CSD$ metric is:
% % \begin{equation}
% $CSD = \sum_{i=1}^n ncn_{i} * k$.
% % \end{equation}
% Note that as lower the value of $CSD$ is for a given program, the better the CFI policy 
% is. The optimal value of this metric is equal to the total number of indirect callsites present 
% in the hardened program when $k$ equals one. The value of $k$ can take any millisecond value.

%
%%put afterwards in appendix
% \begin{definition}[\textbf{RSD}]
%  Let $nrn_{i}$ be the runtime cost for a CFI check performed before an indirect return site $irs_{i}$ which
%  is present in a given hardened program. 
%    Let $k$ be the runtime overhead (damping ratio) imposed by one inserted CFI check at the $irs_{i}$.
%   The $k$ value could represent milliseconds needed to perform a CFI check.
% \label{rsd definition.}
% \end{definition}
% Then the $RSD$ metric is:
% % \begin{equation} 
% $RSD = \sum_{i=1}^n nrn_{i} * k$.
% % \end{equation}
% Note that the lower the value of $RSD$ is for a given program, the better the CFI policy 
% is. The optimal value of this metric is equal to the total number of indirect callsites present 
% in the hardened program when $k$ equals one. The value of $k$ can take any millisecond value.

%

\begin{definition}[\textbf{fCGA}]
Let $cgf_{i}$ be the total number of legitimate
call targets that are allowed and which contain gadgets according to a gadget finding tool. 
\label{fcga definition.}
\end{definition}
Then the forward code reuse gadget availability $fCGA$ metric is:
% \begin{equation}
$fCGA = \sum_{i=1}^n cgf_{i}$.
% \end{equation}
Note that the lower the value of $fCGA$ is, the better the policy is. This means that
every time a calltarget containing a code reuse gadget is protected by a CFI check, this gadget is not reachable. 
The reverse is true when the calltarget return contains a gadget and there
are indirect control flow transfers which can call this indirect return site unconstrained.

%

\begin{definition}[\textbf{bCGA}]
Let $cgr_{i}$ be the total number of legitimate
callee returns addresses which contain code gadgets according to a gadget finding tool. 
\label{bcga definition.}
\end{definition}
Then the backward code reuse gadget availability $bCGA$ metric is:
% \begin{equation}
$bCGA = \sum_{i=1}^n cgr_{i}$.
% \end{equation}
Note that the lower the value of $bCGA$ is, the better the policy is. This means that
every time when a calltarget return site which contains a code reuse gadget is protected by a CFI check then 
this gadget is not reachable. The reverse is true, when the calltarget return contains a gadget and there
are indirect control flow transfers which can call this indirect return site unconstrained.

Above, we depicted these metrics to point out that all these CFI-related measurements
are relevant and could be performed depending on the type of CFI policy a certain tool implements.
The eight assessed CFI policies can neither constrain the backward edge nor analyze their availability
of gadgets and their runtime cost.

The metrics presented above, can be used by \sysname to assess CFI policies w.r.t. other dimensions (\textit{i.e.,} (1) backward edges, and (2) gadget availability)
with which most of the CFI techniques are not addressing.
Thus, we did not use the four metrics in conjunction with the eight CFI classes
assessed in this paper since these metrics to not address (1) and (2).
Moreover, we are not aware of any CFI policy which is based on these
types of four metrics. Finally, we think that by using these metrics experiments
become more reproducible and the tools better comparable against each other.


==> parts/applications.tex <==
We will next present some applications of our ICFI framework.

\subsection{Quantifying Protection Level}
The metrics derived with the help of ICFI help to precisely quantify the protection level offered by a given 
policy for the following reasons. 
First, the metrics are not proving average values. Second, take into consideration the number of locations where a 
certain policy was enforced and where not. Third, the precision of call target or return target set per ics or irt is 
aware of the gaps or the imprecision which is introduced due to an imprecise analysis.

\subsection{Quantifying Damping Level}
ICFI can be used to assess a CFI based policy also from the runtime overhead introduced due to the fact that we consider costs 
for performing a single CFI check before each indirect control flow transfer. Also the ICFI policy considers the 
number of checks that have to be performed before each indirect control flow transfer individually and as such the overall cost 
of each indirect control flow transfer can be assessed. The final outcome is the possibility to provide an exact number of the 
total damping that a CFI policy incurs to any hardened program. Further, these results can be used to asses in more detail if
the policy should be assessed at all or even partially to certain parts of the program. For example certain parts could 
remain unprotected (hot code) in cases where this makes sense in order to strike a balance between the protection level and the 
overall runtime damping of the program.

\subsection{Quantifying Gadget Availability}
The ICFI provided formulas help to assess which indirect control flow transfers should be protected and which not. Since
it is not worthwhile protecting all indirect control flow transfers inside a program since not all
call targets (virtual functions) contain COOP gadgets. Thus, not usable for an attacker. Finally, this metrics help to further 
fine tune towards the decision where to apply check and were these can be left out. The final outcome is a possibility to better
reason about a more reduced runtime overhead. This is in our opinion not negligible when for example we can safely exclude to protect 
indirect control flow transfers which reside in hot code.

\subsection{Quantifying Gadget Link-ability}
As the ICFI policies can be used to assess COOP gadget availability we can also further support reasoning about gadget link-ability.
Since gadget link-ability depends directly on the availability of gadgets our metrics can be used to measure how easy or hard is to 
assemble a certain gadget chain due to the presence or absence of certain gadgets inside a program. 
Also in the case of not protecting all gadgets due to the fact that they can reside in hot we can also further reason about the chances
to successfully assemble a certain chain of gadgets, purely reasoning about the availability of gadgets that were left off unprotected.

==> parts/attacks.tex <==
Here we show how \sysname bypasses a state-of-the-art CFI policy based defense.
This case study is architecture independent, since \sysname's analysis is performed at the IR level during LTO time in LLVM.
Note that LLVM IR code represents a higher level representation of machine code (metadata), thus
our results can be applied to other architectures (\textit{e.g.,} ARM) as well.
Our case study assumes an ideal implementation of VTV/IFCC. Breaking
the ideal instrumentation shows that the defense can be bypassed in any
implementation.

\subsection{Sub-hierarchy Policy (VTV)}
In this case study, we %will not present a full attack as other do but rather start by 
present the required
components for a COOP attack by studying the original COOP attack against Firefox and 
by demonstrating that such an attack is easier to perform with \sysname at hand.

The original COOP attack presented by Schuster \textit{et al.} \cite{coop} used:
(1) a buffer overflow filled with six fake counterfeit objects by the attacker,
(2) precise knowledge of the Firefox \texttt{libxul.so} layout,
(3) where an COOP dispatcher gadget (\texttt{ML-G}) resides, and
(4) several other useful gadgets the attacker was able to open an Unix shell.

In general terms, to pursue a CRA the attacker needs: 
(1) an exploitable memory corruption,
(2) attack starting point (\textit{i.e.,} callsite) becomes corruptible due to (1),
(3) program binary memory layout leak,
(4) appropriate (usable and available) gadgets,
(5) the possibility to read and write into memory,
(6) the possibility to link gadgets and pass information from one to each other, and 
(7) the possibility to perform calls into the system \texttt{stdlib} or any other reach functionality library.

As demonstrated, the attacker has to find first an exploitable memory corruption (\textit{e.g.,} buffer overflow) and fill it with fake objects.
Next the attacker makes calls to different gadgets (virtual functions) located in the program binary. 
As such, we assume that NodeJS contains an exploitable memory vulnerability (\textit{i.e.,} buffer overflow), and that the attacker 
is aware of the layout of the program binary. Next the attacker wants to bend the control flow to only the per callsite legitimate 
calltargets since he does not know which other defenses are in place. Further, he wants to avoid calling into other program
class hierarchies. For this reason, he needs to know which are the legitimate calltargets for all callsites in the main NodeJS binary.
\vspace{.3cm}

\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
 \begin{tabular}{ l | p{.2cm} | p{1.1cm} |  p{1.1cm} | p{.8cm} | p{.6cm} | p{.6cm} | p{.9cm} | p{1.1cm} | p{.8cm} | p{1.2cm} | p{1cm}} \hline
         \multicolumn{1}{c|}{\hspace{.1cm}\textit{\textbf{Controllable}}} &\multicolumn{1}{c|}{}  &\multicolumn{1}{c|}{} &\multicolumn{1}{c|}{}                         & \multicolumn{8}{c}{\hspace{0cm}\textbf{Targets}} \\
         \textit{\hspace{1cm}\textbf{Callsite}}      & \textit{\#}         &\textit{Baseline only vFunc.}    &\textit{Baseline all Func.}          & \textit{Bin types}  & \textit{Safe src types} & \textit{Src types} & \textit{Precise src types} & \textit{All vtables}  & \textit{vtable hierarchy}        & \textit{Sub-hierarchy}  &\textit{Precise Sub-hierarchy}    \\ \hline
         1. debugger.cpp:1329:33                     & 5                   & 6,300                           & 32,478                              & 31,305              &4                        &4                   &1                           &6,128                  &1                                 &1                        &1                                 \\
         2. protocol.cpp:839:60                      & 2                   & 6,300                           & 32,478                              & 21,950              &719                      &719                 &49                          &6,128                  &57                                &53                       &49                                \\
         3. schema.cpp:133:33                        & 3                   & 6,300                           & 32,478                              & 27,823              &136                      &136                 &1                           &6,128                  &1                                 &1                        &1                                 \\
         4. handle\_wrap.cc:127:3                    & 1                   & 6,300                           & 32,478                              & 12,545              &810                      &810                 &1                           &6,128                  &72                                &12                       &12                                \\
         5. cares\_wrap.cc:642:5                     & 1                   & 6,300                           & 32,478                              & 1,956               &810                      &810                 &1                           &6,128                  &72                                &13                       &13                                \\
         6. node\_platform.cc:25:5                   & 1                   & 6,300                           & 32,478                              & 1,956               &810                      &810                 &6                           &6,128                  &20                                &19                       &19                                \\
         7. node\_http2\_core.h:417:5                & 3                   & 6,300                           & 32,478                              & 1,956               &810                      &810                 &6                           &6,128                  &20                                &19                       &19                                \\
         8. tls\_wrap.cc:771:10                      & 2                   & 6,300                           & 32,478                              & 3,106               &35                       &35                  &8                           &6,128                  &48                                &13                       &5                                 \\
         9. protocol.cpp:839:60                      & 2                   & 6,300                           & 32,478                              & 3,106               &2,984                    &2,984               &49                          &6,128                  &53                                &53                       &49                                \\
        10. protocol.cpp:836:60                      & 2                   & 6,300                           & 32,478                              & 3,106               &719                      &719                 &49                          &6,128                  &53                                &53                       &19                                \\
\end{tabular}
}
\caption{Ten controllable callsites and legitimate targets.}
\label{Controllable callsites.}
\end{table}

\autoref{Controllable callsites.} depicts ten controllable callsites (in total \sysname found hundreds of controllable callsies) for which 
the legitimate target set, depending on the used CFI policy, ranges from one to \numprint{31,305} calltargets. 
\# depicts the number of passed parameters.
% \mat{This should be a caption.
For each calltarget \sysname provides: file name, function name, start address, source code line number such that it can be easily 
traced back in the source code file.
The calltargets (right hand side in \autoref{Controllable callsites.} in
italic font) represent available calltargets for each of the eight assessed
policies.

For our case study, we decide not to use the most restrictive CFI policy (\textit{i.e.,} \textit{Precise sub-hierarchy})
as this enforces the same function in the virtual table sub-hierarchy. As such only through inheritance the chances are given 
that the implementation of the function may vary from the initial implementation. Thus, the number of useful gadgets 
in this sub-hierarchy is low.

Consequently, we assume that the attacker knows that the NodeJS binary is protected with the 
\textit{Sub-hierarchy} policy. The attacker ranks all callsites depending on the number of usable calltargets. 
By ranking the callsites w.r.t. their residual target set, the attacker wants to know the 
precise functions (calltargets) which are allowed for each callsite. Further, in order to perform the attack, 
he has to access the source code of the application. 
After searching through the source code, he finds several callsites were vector-based object dispatches are performed. 
The attacker, next finds out that in the detected calltargets set there are 
several usable gadgets. Note that for the COOP attack to be performable the only hard constraint is that at least one usable 
\texttt{ML-G} gadget exists in the program. This constraint was addressed by the attacker at the beginning of her source code search since he decided 
to look for only callsites which are part of an \texttt{ML-G} COOP gadget. As such, the attacker knows exactly which gadgets are available for each controllable callsite. 
As none of the static CFI policies impose write constraints by default (\textit{i.e.,} none) the attacker can overflow a buffer at a certain callsite with fake 
objects. Further, he starts to call his gadgets one by one and passes information over the stack through scratch register from one gadget to the next one.
Note that her attack does not violate the CFI check in place at the selected object dispatch location since this is contained in a \texttt{ML-G} gadget.
Further, he deliberately avoids to violate the original program control flow by calling into other program class hierarchies or other 
illegitimate calltargets as the original COOP attack does. 
Finally, at the end, the attacker succeeds in opening an Unix shell as in the original COOP attack.

This CRA shows that by using \sysname an attacker
can discover which gadgets are legitimate for each callsite after a certain CFI policy was applied in order 
to better tailor her attack w.r.t. a deployed CFI-based defense.


==> parts/formalization.tex <==
\newsavebox{\firstlisting}
\begin{lrbox}{\firstlisting}
\begin{minipage}[c]{\columnwidth}
\begin{minted}[
% frame=lines,
framesep=2mm,
linenos,
highlightlines={10-14, 22-24},
highlightcolor={lightgray},
frame=none,
firstnumber=1,
framesep = .8cm,
linenos,
numbersep=1pt,
%gobble=2,
%frame=lines,
framesep=2mm,
% fontsize=\tiny,      
fontsize=\scriptsize,
% baselinestretch=1.2,
% bgcolor=LightGray,
% fontsize=\footnotesize
]{C++}
class Car {
 public:
  virtual ~Car() { }
  virtual void driverless();
};

class ElectricCar : public virtual Car {
 public:
          bool rechargeElectically(int p1, float p2);
  virtual void accelerateQuietly(int nTimeStamps){
          for (size_t i = 0; i < nTimeStamps; i++)
          timeStamps[i]->setNewSpeed();         
          delete timeStamps;            
  }                                           /*ML-G*/
};

class PetrolCar : public virtual Car {
 public:
 size_t levelNOXold;
 size_t levelNOXnew;
         bool rechargePetrol(double p1);
 virtual int produceNitrogenOxides(int levelNOXnew){
     levelNOXnew = levelNOXnew + levelNOXold;  
 return levelNOXnew;                      /*ARITH-G*/
 }  
};

// A hybride car is still an electric car
class HybrideCar : public PetrolCar, 
                   public ElectricCar {
};
\end{minted}
\end{minipage}
\end{lrbox}

In this section we first introduce the used notation and than the theorems and definitions which are the core 
of the ICFI reasoning framework. 
The goal of this section is to derive our ICFI reasoning framework
which is will be use to prove our assumptions made in the background section.
The framework is based on some definitions
which we will will use afterwards to derive our CFI policy based criterion C++ class slicing algorithm.
Next we derive six metrics which are the core of ICFI by combining the following concepts:
(1) indirect call sites,
(2) class hierarchy,
(3) control flow graphs,
(4) virtual table hierarchies,
(5) virtual table inheritance, and 
(6) counterfeit object-oriented gadgets. 

 \begin{figure}[H]
   \hspace{.1cm}
   \usebox{\firstlisting}
% \caption{Description of how a counterfeit object-oriented programming main loop gadget (ML-G) works.}
\caption{Multiple inheritance class hierarchy.}
\label{Multiple inheritance class hierarchy.}
\end{figure}

\autoref{Multiple inheritance class hierarchy.} depicts a simple C++ class hierarchy with multiple inheritance which we will use as running example in order to 
better convey the theory developed in this paper.
Before starting with the formalization we want to point out several key decisions made.
First, note that the ICFI theory builds on top of the Tip et al.~\cite{class:slicing} extension of the Rosie-Friedman Framework~\cite{rossie:friedman}.
Second, ICFI's goal is to help to measure the level of protection offered by different forward-edge and backward-edge CFI-based protection techniques.
Third, the notation which we will use throughout this section is in our opinion most appealing to research colleagues and has a low understandability bound.
Fourth, we keep our formalizations as close as possible to the natural language such that the understandability boundary is low, we hope that this facilitates fast adoption of the ideas presented herein.
Finally, all definitions and theorems presented next are related to the C++ language N4296~\cite{N4140} and to the the COOP~\cite{coop} attack.

\subsection{ICFI Notation}
\label{ICFI notation}
For details about the notation used in this paper refer to~\cite{class:slicing}. In this paper we refer to class members
as indirect control flow transfer targets. These are stemming similar as in~\cite{class:slicing} from object dispatches when 
considering only forward edges. Further, note that by having a precise relation on the legitimate forward edges (i.e., class hierarchy enforcement)
one can derive a relation for the legitimate backward edges to the return addresses as well (e.g., by reflecting the class hierarchy 
back from the calltarget returns to the addresses next to each legitimate callsite).

\subsection{ICFI Formalization}
\subsubsection{Extended Class Hierarchy Definition}
Our class hierarchy definition is based on the class definition of Tip et al.~\cite{class:slicing}.
Let $\mathcal{C}$ be the set of class names, $\mathcal{M}$ denote the set of member names. 
We assume that the class names are unique and that a sort of naming convention is in place.
$\mathcal{V}$ denote the set of \{virtual, non-virtual\}. 
Additionally, let $\mathcal{O}$ denote the set of \{parameterCount, parameterTypes, returnType\}. 
The class hierarchy can be defined as follows.

\begin{definition}
\label{Extended Class Hierarchy}
A class $\gamma$ is a tuple $\langle$\^{C}, \^{M}, \^{P}, \^{S}$\rangle$  where:
\begin{itemize}
 \item[(1)] \^{C} $\subseteq$ $\mathcal{C}$, 
 \item[(2)] \^{M} $\subseteq$ \^{C} $\times$ $\mathcal{M}$ $\times$ $\mathcal{V}$ $\times$ $\mathcal{O}$, 
 \item[(4)] \^{S} $\subseteq$ \^{C} $\times$ \^{C}, and 
 \item[(5)] \^{P} $\subseteq$ \^{C} $\times$ \^{C} such that: 
 \begin{itemize}
  \item[(i)] \^{S} and \^{P} are irreflexive,
  \item[(ii)] \^{S} $\cap$ \^{P} = $\emptyset$, 
  \item[(iii)] the transitive closure of \^{S} $\cup$ \^{P} is antisymmetric,
  \item[(iv)] if (X, m, $f_{1}$, p, t, r$\rangle$  $\in$ \^{M} and (X, m, $f_{2}$, p, t, r$\rangle$  $\in$ \^{M} then $f_{1}$ = $f_{2}$, and
  \item[(v)] if (X, m, virtual, p, t, r$\rangle$  $\in$ \^{M}, (Y, m, f, p, t, r$\rangle$  $\in$ \^{M}, and (Y, X) $\in$ (\^{S} $\cup$ \^{P})* then f = virtual.
  \item[(vi)] if (X, $m_{1}$, $f_{1}$, p1, t1, r$\rangle$  $\in$ \^{M} and (X, $m_{2}$, $f_{2}$, p2, t2, r) $\in$ \^{M} and $f_{1}$ = $f_{2}$ and $m_{1}$ = $m_{2}$ and t1 = t2 then p1 = p2,
  \item[(vii)] if (X, $m_{1}$, $f_{1}$, parameterCount1, parameterTypes1, r1$\rangle$  $\in$ \^{M} and (X, $m_{2}$, $f_{2}$, parameterCount2, parameterTypes2, r2$\rangle$  $\in$ \^{M} and $f_{1}$ = $f_{2}$ and $m_{1}$ = $m_{2}$ 
       and p1 = p1 and t1 = t2 and r1 = r2 then (X, $m_{1}$, $f_{1}$, p1, t1, r1$\rangle$  = (X, $m_{2}$, $f_{2}$, p2, t2, r2$\rangle$ .
 \end{itemize}
\end{itemize}
\end{definition}

For a given class hierarchy $\gamma$, its components are denoted by 
\^{C}($\gamma$), \^{M}($\gamma$), \^{S}($\gamma$), \^{P}($\gamma$), respectively.
The reflexive and transitive closure of (\^{S} $\cup$ \^{P}) will be denoted by
\^{I}($\gamma$). For ((i) to (v) see ~\cite{class:slicing}). 
Additionally, (vi) two members which can not be virtual and non-virtual at the same time, which have the same name and the same types set then these members have the same parameter count set,
(vii) two members which can not be virtual and non-virtual at the same time, which have the same name, the same parameter set count and
the same ordered parameter set type and have the same return type type are the same. Such members are unique in the class hierarchy.

\begin{example}
From \autoref{Extended Class Hierarchy} it follows that for the program depicted in \autoref{Multiple inheritance class hierarchy.} 
we have the class hierarchy.
\end{example}

{\footnotesize
\begin{subequations}
\begin{align*}
{\hat C}(\gamma) =& \{Car, ElectricCar, PetrolCar, HybrideCar\} \\
{\hat M}(\gamma) =& \{\langle Car, driverless, virtual, 0, (void), void\rangle,\\
                  &  \langle ElectricCar, accelerateQuietly, virtual, 1, (int), void\rangle, \\
                  &  \langle ElectricCar, rechargeElectically, nonvirtual, 2, (int, \\ 
                  &   float), bool\rangle, \\
                  &  \langle PetrolCar, produceNitrogenOxides, virtual, 1, (int), int\rangle,\\
                  &  \langle PetrolCar, rechargePetrol, non\-virtual, 1, (double), bool\rangle\}\\
{\hat S}(\gamma) =& \{\langle ElectricCar, Car\rangle, \\
                  &   \langle PetrolCar, Car\rangle\}\\
{\hat P}(\gamma) =& \{\langle HybrideCar, ElectricCar\rangle, \\
                  &   \langle HybrideCar, PetrolCar\rangle\}
\end{align*}
\label{Class hierarchy path.}
\end{subequations}}

\subsubsection{Class Hierarchy Path}
A class hierarchy path is based on the class Definition~\autoref{Extended Class Hierarchy}. 
Additionally class inheritance is taken into account and paths
are formed between virtual and non-virtual members each taken into 
the chain of relations once.

\begin{definition}
\label{Class hierarchy path}
 A class hierarchy path is a 5-tuple $\langle$\^{C}, \^{M}, \^{P}, \^{S}, \^{T}$\rangle$  where:
 \begin{itemize}
 \item[(1)] all the relations defined in the class Definition~\autoref{Extended Class Hierarchy} still hold.
 
 \item[(2)] \^{T} represent any possible simple path with no cycle between any two members from \^{C}.
 Thus any path contains at least two members from \^{C}.
 Further, each element in \^{T} is unique and the path nodes contain:
 \begin{itemize}
  \item[(i)] non-virtual statically defined members,
  \item[(ii)] virtual statically defined members,
  \item[(iii)] non-virtual dynamically inherited members, and 
  \item[(iv)] virtual dynamically members which are available as a consequence of class inheritance during runtime.
 \end{itemize}
 \end{itemize}
\end{definition}

\begin{example}
From Definition~\autoref{Class hierarchy path} it follows that for the program depicted in \autoref{Multiple inheritance class hierarchy.} 
we have the class hierarchy path.
\end{example}

{\footnotesize
\begin{subequations}
\begin{align*}
{\hat C}(\gamma) =& \{Car, ElectricCar, PetrolCar, HybrideCar\} \\
{\hat M}(\gamma) =& \{\langle Car, driverless, *virtual*\rangle ,\\
                  &  \langle ElectricCar, accelerateQuietly, *virtual*\rangle, \\
                  &  \langle ElectricCar, rechargeElectically, *nonvirtual*\rangle, \\
                  &  \langle PetrolCar, produceNitrogenOxides, *virtual*\rangle ,\\
                  &  \langle PetrolCar, rechargePetrol, *non-virtual*\rangle \}\\
{\hat S}(\gamma) =& \{\langle ElectricCar, Car\rangle, \\
                  &   \langle PetrolCar, Car\rangle  \}\\
{\hat P}(\gamma) =& \{\langle HybrideCar, ElectricCar\rangle, \\
                  &   \langle HybrideCar, PetrolCar\rangle \}\\
{\hat T}(\gamma) =& \{\langle Car, ElectricCar \rangle,\\
                  &   \langle Car, ElectricCar, HybrideCar \rangle,\\  
                  &   \langle ElectricCar, HybrideCar \rangle,\\  
                  &   \langle Car, PetrolCar \rangle ,\\  
                  &   \langle Car, PetrolCar, HybrideCar \rangle, \\
                  &   (PetrolCar, HybrideCar \rangle\}  
\end{align*}
\label{Class hierarchy path.}
\end{subequations}}

Note that each of the paths contained in ${\hat T}(\gamma)$ is a subset of ${\hat M}(\gamma)$ w.r.t. the 
number of calltargets contained. Further, a path is a subset of the class hierarchy, 
${\hat T}(\gamma) \subset \mathcal{C}$. Thus $CH_{path} \subseteq CH$.
% This definition proves that \cref{CH path subset of CH} holds.

\subsubsection{Virtual Table Subhierarchy}
According to Definition 4.3~\cite{class:slicing} it follows that for any
two class subhierarchies $\gamma$ and $\gamma$' the following holds.
$\gamma$' is a subhierarchy of $\gamma$ ($\gamma$' $\sqsubseteq$ $\gamma$) $iff$ 
\begin{itemize}
\item [(i)] ${\hat V}$($\gamma$)' $\subseteq$ ${\hat C}$($\gamma$)
\item [(ii)] ${\hat V}$($\gamma$)' $\subseteq$ ${\hat M}$($\gamma$)
\item [(iii)] ${\hat V}$($\gamma$)' $\subseteq$ ${\hat P}$($\gamma$)
\item [(iv)] ${\hat V}$($\gamma$)' $\subseteq$ ${\hat S}$($\gamma$)
\end{itemize}

From this definition we observe that two class subhierarchies 
are subhierarchies of each other if the set of members of the first 
subhierarchy is a subset of set of members of the second subhierarchy (ii)
and (i), (iii), and (iv) hold. Next we will give the definition of a
virtual table hierarchy.

\begin{definition}
\label{Virtual Table Hierarchy Definition}
A virtual table hierarchy $\beta$ is a 4-tuple $\langle$ ${\hat V}_{C}$, ${\hat V}_{M}$, ${\hat V}_{P}$, ${\hat V}_{S}$ $\rangle$ where:
\end{definition}

\begin{itemize}
\item[(1)] ${\hat V}_{C}$ $\subseteq$ $\mathcal{C}$, 
\item[(2)] ${\hat V}_{M}$ $\subseteq$ \^{C} $\times$ $\mathcal{M}$ $\times$ $\mathcal{V}$, 
\item[(3)] ${\hat V}_{S}$ $\subseteq$ \^{C} $\times$ \^{C}, and 
\item[(4)] ${\hat V}_{P}$ $\subseteq$ \^{C} $\times$ \^{C} such that: 
 \begin{itemize}
  \item[(i)] ${\hat V}_{S}$ and ${\hat V}_{P}$ are irreflexive,
  \item[(ii)] ${\hat V}_{S}$ $\cap$ ${\hat V}_{P}$ = $\emptyset$, 
  \item[(iii)] the transitive closure of ${\hat V}_{S}$ $\cup$ ${\hat V}_{P}$ is antisymmetric,
  \item[(iv)] if $\langle$ X, m, $f_{1}$ $\rangle$  $\in$ ${\hat V}_{M}$ and $\langle$ X, m, $f_{2}$ $\rangle$  $\in$ ${\hat V}_{M}$ then $f_{1}$ = $f_{2}$, and
  \item[(v)] if $\langle$ X, m, *virtual*$\rangle$  $\in$ ${\hat V}_{M}$, $\langle$ Y, m, f$\rangle$  $\in$ ${\hat V}_{M}$, and $\langle$ Y, X$\rangle$  $\in$ $\langle$ ${\hat V}_{S}$ $\cup$ ${\hat V}_{P}$ $\rangle$ * then f = *virtual*.
 \end{itemize}
\end{itemize}

For a given *virtual* table hierarchy $\beta$, its components are denoted by 
${\hat V}_{C}$($\beta$), ${\hat V}_{M}$($\beta$), ${\hat V}_{S}$ ($\beta$), ${\hat V}_{P}$($\beta$), respectively.
The reflexive and transitive closure of ${\hat V}_{S}$ $\cup$ ${\hat V}_{P}$) will be denoted by ${\hat V}_{I}$($\beta$).
${\hat V}_{M}$ contains only *virtual* members.


Consider the definition of a *virtual* table hierarchy similar to the definition of the 
class hierarchy only that the members contained in
\^{M} are only *virtual* functions. The *virtual* table hierarchy can be considered a slice 
of a class hierarchy containing only *virtual* members.

Since a *virtual* table hierarchy contains only *virtual* members than it is a subset of 
the class hierarchy which contains *virtual*, non-*virtual* and other member types. 
Then the following relation holds $\beta$ $\subseteq$ $\gamma$. 
% This definition proves 
% that \cref{VTH path subset of CH} ($VTH \subseteq CH$) holds.

\begin{example}
From Definition~\autoref{Virtual Table Hierarchy Definition} it follows that for the program depicted in~\autoref{Multiple inheritance class hierarchy.} 
we have the virtual table hierarchy $\beta$.
\end{example}

{\footnotesize
\begin{subequations}
\begin{align*}
{\hat V}_{C}(\beta) =& \{Car, ElectricCar, PetrolCar, HybrideCar\}\\
{\hat V}_{M}(\beta) =& \{\langle Car, driverless, *virtual*\rangle ,\\
                     &   \langle ElectricCar, accelerateQuietly, *virtual*\rangle, \\
                     &   \langle PetrolCar, produceNitrogenOxides, *virtual*\rangle \}\\
{\hat V}_{S}(\beta) =& \{\langle ElectricCar, Car\rangle , \langle PetrolCar, Car\rangle \}\\
{\hat V}_{P}(\beta) =& \emptyset
\end{align*}
% \label{Virtual table hierarchy.}
\end{subequations}}

\subsubsection{Virtual Table Hierarchy Path}
A virtual table hierarchy path is based on the \cref{Virtual Table Hierarchy Definition}.
The main difference between class paths and virtual paths is that the virtual 
paths contain only virtual table entries.

\begin{definition}
\label{virtual table hierarchy path}
 A virtual table hierarchy path is a 5-tuple $\langle$\^{C}, \^{M}, \^{P}, \^{S}, \^{T}$\rangle$  where:
 \begin{itemize}
 \item[(1)] all the relations defined in the class Definition~\autoref{Extended Class Hierarchy} still hold.
 
 \item[(2)] \^{T} represent any possible simple path with no cycle between any two members from \^{C}.
 Thus any path contains at least two members from \^{C}.
 Further, each element in \^{T} is unique and the path nodes contain only:
 \begin{itemize}
  \item[(i)] virtual statically defined members, and
  \item[(ii)] virtual dynamically members which are available as a consequence of class inheritance during runtime.
 \end{itemize}
 \end{itemize}
\end{definition}

\begin{example}
For example from Definition~\autoref{virtual table hierarchy path} it follows that for the 
program depicted in~\autoref{Multiple inheritance class hierarchy.} 
we have the following virtual table hierarchy path.
\end{example}

{\footnotesize
\begin{subequations}
\begin{align*}
{\hat C}(\beta) =& \{Car, ElectricCar, PetrolCar, HybrideCar\} \\
{\hat M}(\beta) =& \{\langle Car, driverless, *virtual*\rangle ,\\
                  &  \langle ElectricCar, accelerateQuietly, *virtual*\rangle , \\
                  &  \langle PetrolCar, produceNitrogenOxides, *virtual*\rangle\} \\
{\hat S}(\beta) =& \{\langle ElectricCar, Car\rangle , \\
                  &   \langle PetrolCar, Car\rangle  \}\\
{\hat V}_{P}(\beta) =& \emptyset \\
{\hat T}_{vpath}(\beta) =& \{\langle ElectricCar, HybrideCar \rangle ,\\ 
                  &    \langle PetrolCar, HybrideCar \rangle \}  
\end{align*}
% \label{Virtual table hierarchy path.}
\end{subequations}}

Note that $HybrideCar$ which has no static inherited functions is contained in ${\hat M}(\beta)$
since it will have virtual members available during runtime as a consequence of inheritance.
Note that the class $Car$ can not be included in any path since it has no virtual members declared inside.
Note that ${\hat M}(\beta)$ is a subset of ${\hat M}(\gamma)$ from \cref{Virtual Table Hierarchy Definition}
w.r.t. the number of calltargets contained (members). 
Further, since the virtual table hierarchy path contains less members than 
class paths the set ${\hat T}_{vpath}(\beta) \subseteq {\hat T}_{path}(\beta)$. 
It results that $VTH_{path} \subseteq CH$, but $VTH \subseteq CH$, thus 
$VTH_{path} \subseteq VTH$. 
% This definition proves that \cref{VTH path subset of VTH} holds.

\subsubsection{Gadgets and Virtual Table Hierarchies}
A code reuse gadget $crg$ is a sequence of machine instructions with variable length 
containing typically a part, an $bb$, or multiple $bb$ which end in an indirect instruction $ii$.
An $ii$ is typically used during CRAs to exploit the imprecision which 
can not be precisely handled during checking when $ie$ are used.

In case of the COOP attack a gadget ($cg$) is a member in the $CH$. Since the $VTH \subseteq CH$ this means that 
$cg$ is a member contained in $VTH$. COOP gadgets are virtual functions, thus each $cg$ is contained in ${\hat S}(\beta)$.

A COOP gadget $cg$ is not necessarily a linear set of machine instructions which contains one or more $bb$ and which originates from exactly 
one $vtbl$ entry contained in the $vtbl$ and which corresponds to one class member.
A $cg$ is available inside $P$ to an attacker $A$ if between the $ie$ which connects during runtime a particular $ics$ with a $ct$ no 
type of runtime CFI based check is enforced.
A $cg$ is not available inside $P$ to $A$ if between the indirect $cfg$ edge which connects during runtime a particular $ics$ with a $ct$ at 
least one runtime CFI based check is enforced.
We say that the set of available $ct$ per $ics$ is \textit{constrained} when a particular runtime CFI based check is enforced during runtime for each $ie$.
The ideal set enforces a 1:1 mapping between each $ics$ and $ct$.
The most strict type of check which can be enforced for a particular $ics$ is based on the $MinVTable_{path}$.
The $MinVTable_{path}$ is determined by the longest virtual table inheritance path determined between the base class of the object making the dispatch and
a leaf node in the virtual table hierarchy.

% \begin{proof}
% Evident: common knowledge. The minimal set of virtual tables that should be allowed per $ics$ is determine by the longest virtual table inheritance path
% which starts at the class type of the object responsible for the $ics$ and terminates at one of the leaf nodes inside the $qt$. 
% See ShrinkWrap~\cite{shrinkwrap}  paper for a practical GCC based implementation of this concept.
% \end{proof}

\begin{definition}
\label{coop gadget set definition}
A gadget set $\alpha$ is a 3-tuple $\langle$ ${\hat G}_{types}$, ${\hat G}_{attributes}$, ${\hat G}_{set}$ $\rangle$  where:

\begin{itemize}
 \item[1)] ${\hat G}_{set}$ is included in the class hierarchy of a given program.
 \item[2)] ${\hat G}_{set}$ is included in the virtual table hierarchy of a given program.
 \item[3)] ${\hat G}_{set}$ contains only the virtual functions which have their type defined in ${\hat G}_{types}$.
 \item[4)] all elements contained in ${\hat G}_{set}$ are available to an attacker if no CFI-based policy was applied.
 \item[5)] the elements of ${\hat G}_{set}$ are called only trough corrupted object dispatches.
 \item[6)] the size of ${\hat G}_{types}$ has a fixed size (e.g., for the COOP attack it is 10).
\end{itemize}

\end{definition}

\begin{example}
 From Definition~\autoref{coop gadget set definition} it follows that for the program depicted in~\autoref{Multiple inheritance class hierarchy.} 
 we have the following $\alpha$.
\end{example}

{\footnotesize
\begin{subequations}
\begin{align*}
{\hat G}_{types}(\beta) =& \{ML \mymathhyphen G, ARITH \mymathhyphen G, W \mymathhyphen G, R \mymathhyphen G, INV \mymathhyphen G, \\
                         & W \mymathhyphen COND \mymathhyphen G, ML \mymathhyphen ARG \mymathhyphen G, W \mymathhyphen SA \mymathhyphen G, \\ 
                         & MOVE \mymathhyphen SP \mymathhyphen G, LOAD \mymathhyphen R64 \mymathhyphen G  \} \\
{\hat G}_{attributes}(\beta) =& \{function \mymathhyphen signature, startMemoryAddress, \\
                              &usable, not \mymathhyphen usable, type \} \\
{\hat G}_{set}(\beta) =& \{\langle accelerateQuietly, 232121, usable, ML \mymathhyphen G \rangle , \\
                       & \langle produceNitrogenOxides, 347843, usable, \\
                       & ARITH\mymathhyphen G \rangle \}\\
\end{align*}
\label{Gadget set for the COOP attack.}
\end{subequations}}

\autoref{Gadget set for the COOP attack.} depicts the gadget set for the COOP attack.

Note that the COOP gadgets are all virtual functions and as such members in the $VTH$. Due to the fact that not all
gadgets contained in a program P are usable to an attacker we have that $CG_set \subseteq VTH$. 
% This confirms the assumption from the \cref{CG set is subset of VTH}.

  
\subsection{CFI Policy based Class Slicing Algorithm}
In this section we introduce our CFI policy based class slicing Algorithm~\autoref{alg:policy:assessment} and give some CFI policies 
examples which can be assessed with the help of our compiler based tool in order to demonstrate its generality. The goal
of our tool is to provide absolute lower bounds w.r.t. the calltarget and return target set for any given program.
In this way a CFI policy which is program class hierarchy aware can be assessed against each other by counting the minimal set of targets
which it enforces for each program indirect control flow transfer.
Further, in order to asses the available target set per callsite after a CFI policy was applied the following CFI 
policies examples can be assessed against each other by using our tool.

\textbf{Policy1.} Count all legitimate targets in an object dispatch based subhierarchy for all virtual an non virtual members.

\textbf{Policy2.} Count all legitimate targets in an object dispatch based subhierarchy for all virtual members.

\textbf{Policy3.} Count all legitimate targets in an object dispatch based subhierarchy for all virtual members that are COOP gadgets.

\textbf{Policy4.} Count all legitimate targets in an object dispatch determined longest inheritance path containing only virtual members.

\textbf{Policy5.} Count all legitimate targets in an object dispatch determined longest inheritance path containing only virtual members that are COOP gadgets.

\textbf{Policy6.} Count all legitimate targets in an object dispatch based subhierarchy containing virtual members which are expecting up to 6 parameters.

\textbf{Policy7.} Count all legitimate targets in an object dispatch based subhierarchy containing virtual members which are expecting up to 6 parameters and are COOP gadgets.

\textbf{Policy8.} Count all legitimate targets in an object dispatch based subhierarchy containing virtual and non-virtual members which are expecting up to 6 parameters.

\textbf{Policy9.} Count all legitimate targets in an object dispatch based subhierarchy containing virtual and non-virtual members which are expecting up to 6 parameters and are COOP gadgets.

\textbf{Policy10.} Count all targets (legitimate and illegitimate) in a class hierarchy for each object dispatch containing virtual and non-virtual members which are expecting up to 6 parameters.

\textbf{Policy11.} Count all targets (legitimate and illegitimate) in a class hierarchy for each object dispatch containing virtual and non-virtual members which are expecting up to 6 parameters and are COOP gadgets.

 	
\begin{algorithm}[h!]
        \scriptsize
	\SetAlgoLined
	
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{hierarchy, typeSet, Class}
        \Output{SubObjectSet}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{CorrespondingSubobjects}(hierarchy ; TypeSet; Class)}
	{
 	$SubObjSet$ = $\emptyset$        \Comment*[r]{initialize empty set}
 	
 	\ForEach{\text{\upshape class C $\in$ T}}{
 	
 		$SubObjSet$ = $SubObjSet$ $\cup$ \\ \{$\sigma$ | $\sigma$ $\in$ $\sum(\gamma, C)$ and $ldc(\sigma)$ = X\}
	}

	\Return $SubObjSet$              \Comment*[r]{return the sub-object set}

	}
\caption{Get corresponding subobjects}
\label{alg:reaching}
\end{algorithm}

\begin{algorithm}[h!]
        \scriptsize
	\SetAlgoLined
	
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{hierarchy, TypeSet, Class}
        \Output{SubObjectSet}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{GettAllClassObjects}(hierarchy; Class)}
	{
 	$allObjSet$ = $\emptyset$        \Comment*[r]{initialize empty set}
 	
 	//T represents all possible types in the class hierarchy
 	
 	\ForEach{\text{\upshape class C $\in$ ${\hat C}(\gamma)$}}{
 	
 		$allObjSet$ = $allObjSet$ $\cup$ \{$\sigma$ | $\sigma$ $\in$ $\sum(\gamma, C)$\}
	}

	\Return $allObjSet$              \Comment*[r]{return the sub-object set}

	}
\caption{Get all objects in the class hierarchy}
\label{alg:reaching}
\end{algorithm}

\begin{algorithm}[h!]
        \scriptsize
%         \small
%         \footnotesize
	\SetAlgoLined
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{A class hierarchy $\gamma$}
        \Output{CFI policy based measurements}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{CFI\_Policy\_Slicing}(Class: $\gamma$, CFI\_Policy: policy)}
	{
 	
 	\ForEach{\text{\upshape (implicit or explicit) object creation construct $e$ in $\gamma$}}{
 	
 	$instantiatedClasses$ = $instantiatedClasses$ $\cup$ \{class instantiated by $e$\}\;
 	}
 	
 	$\gamma_{slice}$ = $\langle$ $instantiatedClasses$, $\emptyset$, $\emptyset$, $\emptyset$ $\rangle$\;
        
        \ForEach{\text{\upshape (im/ex)plicit typecast expr. $(T*) e$ / $(T\&) e$ / $(T)$ e in $\gamma$}}{
 	
 	$\gamma_{slice}$ = $\gamma_{slice}$ $\cup$ $SubHierClass_{\gamma}(StaticType(e), T)$\;
 	
 	}
 	
 	 $\gamma_{sliceSub}$ = $\gamma_{slice}$;  
 	
 	\textbf{call} $ComputePotentialRuntimeTypes(P)$\; 
 	
 	\ForEach{\text{\upshape implicit or explicit expression} e.m or e$\rightarrow$m in P}{
 	
 	$SubObjectSet$ = $CorrespondingSubobjects(\gamma$, 
 	                                           
 	                                           $\hfill$ $PotentialRunTimeTypes(e)$,
 	                                           
 	                                           $\hfill\hfill\hfill$ $StaticType(e))$\;
 	
 	   
 	\Comment*[l]{get all objects for a class}
 	 
 	 $AllObjectSet$ = $GettAllClassObjects(\gamma$)\;
 	  
 	\Comment*[l]{CFI policies switch case}
 	
        \Switch{$policy$}{
            \Case{$(policy$ = $Policy1)$}{
 	  
 	     \ForEach{$\sigma$ in $SubObjectSet$}{
             
 	      $\gamma_{sliceSub}$ = $\gamma_{sliceSub}$ $\cup$ $MemberLookupSlicePolicy1(\gamma, \sigma, m, n)$;
 	     
 	      $m_{PresentInSlice}$ = $m_{PresentInSlice}$ $\cup$ $countMembers(\gamma_{sliceSub})$;
 	    }

            $totalCalltargets$ = $totalCalltargets$ $+$ $m_{PresentInSlice}$;
                
            }\Case{$(policy$ = $Policy7)$}{
             \ForEach{$\sigma$ in $SubObjectSet$}{
             
 	      $\gamma_{sliceSub}$ = $\gamma_{sliceSub}$ $\cup$ $MemberLookupSlicePolicy7(\gamma, \sigma, m, n)$;
 	     
 	      $m_{PresentInSlice}$ = $m_{PresentInSlice}$ $\cup$ $countMembers(\gamma_{sliceSub})$;
 	    }
           
            
            $totalCalltargets$ = $totalCalltargets$ $+$ $m_{PresentInSlice}$;
            
            }\Case{$(policy$ = $Policy11)$}{
             \ForEach{$\sigma$ in $AllObjectSet$}{
             
 	      $\gamma_{sliceSub}$ = $\gamma_{sliceSub}$ $\cup$ $MemberLookupSlicePolicy11(\gamma, \sigma, m, n)$;
 	     
 	      $m_{PresentInSlice}$ = $m_{PresentInSlice}$ $\cup$ $countMembers(\gamma_{sliceSub})$;
 	    }
           
            
            $totalCalltargets$ = $totalCalltargets$ $+$ $m_{PresentInSlice}$;
            
            }\Other{
            
            \Comment*[l]{implement new policy}
            
            }
            
         }
         
 	}
 	
	\Return $totalCalltargets$              \Comment*[l]{Policy based calltargets}

	}
\caption{CFI Policy Criterion based Class Slicing}
\label{alg:policy:assessment}
\end{algorithm}

\begin{algorithm}[h!]	
	\scriptsize
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{hierarchy $\gamma$; Subobject $\sigma$; member $m$; paramCount $n$}
        \Output{hierarchy}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{MemberLookupSlicePolicy1}($\gamma$; $\sigma$; $m$; $n$; $m_{type}$)}
	{
 	$\sigma' = staticLookup(\gamma, \sigma, m)$        
 	
 	$staticLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
 	                       $\cup$ $SubHier_{\gamma}(\sigma, \sigma')$
 	                       $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, \sigma, m)$\})\; 
 	
 	\Comment*[r]{virtual member lookup}
 	
 	\uIf{(ldc($\sigma'), m, virtual$) $\in$ ${\hat M}(\gamma)$}{ 
             
             $\sigma'$ = dynamicLookup($\gamma, \sigma, m$)
             
             $dynamicLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
                                  $\cup$ $SubHier_{\gamma}([mdc(\sigma), mdc(\sigma)], \sigma')$
 	                          $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, [mdc(\sigma), mdc(\sigma)], m)$\})\;
 	                      
             $lookupSlice$ = $staticLookupSlice$ $\cup$ $dynamicLookupSlice$\;
        }
       
        \Else{
             $lookupSlice = staticLookupSlice$\;
        }
	\Return $lookupSlice$              \Comment*[r]{return the lookup slice}

	}
	
\caption{Get legitimate members.}
\label{alg:reaching}
\end{algorithm}

\begin{algorithm}[h!]	
	\scriptsize
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{hierarchy $\gamma$; Subobject $\sigma$; member $m$; paramCount $n$}
        \Output{hierarchy}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{MemberLookupSlicePolicy7}($\gamma$; $\sigma$; $m$; $n$; $m_{type}$)}
	{
 	$\sigma' = staticLookup(\gamma, \sigma, m)$        \Comment*[r]{initialize empty set}
 	
 	$staticLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
 	                       $\cup$ $SubHier_{\gamma}(\sigma, \sigma')$
 	                       $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, \sigma, m)$\})\; 
 	                    
 	\Comment*[r]{virtual member lookup, with params up to 6 and member are COOP gadgets}
 	
 	\uIf{$\langle$ldc($\sigma'), m, virtual, n\le6, m\in{\hat G}_{types}(\gamma)$$\rangle$ $\in$ ${\hat M}(\gamma)$}{
             
             $\sigma'$ = dynamicLookup($\gamma, \sigma, m$)
             
             $dynamicLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
                                  $\cup$ $SubHier_{\gamma}([mdc(\sigma), mdc(\sigma)], \sigma')$
 	                          $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, [mdc(\sigma), mdc(\sigma)], m)$\})\;
 	                      
             $lookupSlice$ = $staticLookupSlice$ $\cup$ $dynamicLookupSlice$\;
        }
       
	\Return $lookupSlice$              \Comment*[r]{return the lookup slice}

	}
	
\caption{Get legitimate members.}
\label{alg:reaching}
\end{algorithm}

\begin{algorithm}[h!]	
	\scriptsize
	\SetKwInOut{Input}{Input}
        \SetKwInOut{Output}{Output}
        \Input{hierarchy $\gamma$; Subobject $\sigma$; member $m$; paramCount $n$}
        \Output{hierarchy}
        \BlankLine
	\SetKwProg{Fn}{Function}{ is}{end}
	\Fn{\texttt{MemberLookupSlicePolicy11}($\gamma$; $\sigma$; $m$; $n$; $m_{type}$)}
	{
 	$\sigma' = staticLookup(\gamma, \sigma, m)$        
 	
 	$staticLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
 	                       $\cup$ $SubHier_{\gamma}(\sigma, \sigma')$
 	                       $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, \sigma, m)$\})\; 
 	
	\Comment*[r]{virtual member lookup, with params up to 6 and member are COOP gadgets}
 	
 	\uIf{$\langle$ldc($\sigma'), m, virtual, n\le6, m\in{\hat G}_{types}(\gamma)$$\rangle$ $\in$ ${\hat M}(\gamma)$}{
             
             $\sigma'$ = dynamicLookup($\gamma, \sigma, m$)
             
             $dynamicLookupSlice$ = ($\emptyset, \overline{\mathbb{M}}(\gamma, ldc(\sigma'), m), \emptyset, \emptyset$) 
                                  $\cup$ $SubHier_{\gamma}([mdc(\sigma), mdc(\sigma)], \sigma')$
 	                          $\cup$ ($\cup$ \{$SubHier_{\gamma}$($\sigma'$, $\sigma''$) | $\sigma''$ $\in$ $VisibleDefs(\gamma, [mdc(\sigma), mdc(\sigma)], m)$\})\;
 	                      
             $lookupSlice$ = $staticLookupSlice$ $\cup$ $dynamicLookupSlice$\;
        }
       
        \Else{
             $lookupSlice = staticLookupSlice$\;
        }
	\Return $lookupSlice$              \Comment*[r]{return the lookup slice}

	}
	
\caption{Get legitimate members.}
\label{alg:reaching}
\end{algorithm}

% \newpage
\subsection{ICFI Metrics}
In this section we introduce our six metrics which can be used inside our above presented algorithm in order to perform different types of 
measurements.
These six metrics can be used together with our program slicing algorithm in order to determine maximum legitimate call target 
and return target counts for each indirect control flow transfer inside a given program.
We opted for six metrics in order to be able to reason in a more fine grained fashion about the 
protection level offered by a certain CFI-based protection tool. Note that our metrics
do not provide average values but rather absolute numbers and in this way the results from 
different tools can be better compared against each other.

\subsubsection{Indirect Callsite Target Reduction}
We now define our indirect call site target reduction ($iCTR$) 
metric which will be used to measure quantitatively the precise target reduction of
each $ics_{i}$ located inside $P$.

\begin{definition}[\textbf{iCTR}]
Let $ics_{0\_i}$ be a particular indirect call site in $P$,
$ctr_{0\_vi}$ is the total number of available call targets after applying an \textit{ideal} policy 
for all $ics_{0\_i}$ contained in $P$ than the $iCTR$ metric is as follows.
\end{definition}

\begin{equation}
iCTR = \sum_{i=1}^n \sum_{i=j}^m ctr_{0\_i,j}
\end{equation}

Think about \textit{ideal} to be a set of indirect call targets which is determine by the $P$ runtime. This basically means
that each $ics$ has exactly one indirect call target. After all we want to have decidable program execution.
The $iCTR$ is strictly related to each $ics_{i}$ and the values of $ctr_{i}$ and $ctl$ are coupled to $ch$, $vth$ and $vti$.
The lowest value for $iCTR$ for which we have optimal protection is obtained when for each $ics_{i}$ we
have exactly one possible call target. In other words: $iCTR= 1 + 1 + ... + 1 = n $. 
This happens only when there is exactly a 1:1 mapping between each $ics0_{0\_i}$ and $ict_{0\_i,j}$ inside $P$. 
This basically corresponds to the result of the object dispatching mechanism and to the protection of a perfect implemented shadow stack.

In general as closer the value of $iCTR$ is to $n$ the more precise the applied CFI policy is and as higher 
the value of $iCTR$ is w.r.t. $n$ the less precise the used CFI based policy is. Note that in case the value of $ctr_{0\_i}$ is high
this does not influence the security level of the CFI policy only in case the target set is not pure (contains illegitimate call target as a result
of an imprecise analysis). As higher the total number of illegitimate targets added in total the lower the security level is. Note that if
the $ctr_{0\_i}$ high values (basically there are many illegitimate targets in the set) the security level of the policy drops.

\subsubsection{Indirect Returns Target Reduction}
We now define our indirect return site target reduction ($iRTR$) 
formula which will be used to measure quantitatively the precise target reduction of
each $irs_{i}$ for a given $P$.

\begin{definition}[\textbf{iRTR}]
Let $ics_{0\_i}$ be a particular indirect call site in $P$,
$rtr_{0\_i}$ is the total number of available return targets after applying an ideal policy based on a $ch$ for all $ics_{0\_i}$ contained in $P$ than the $iRTR$ metric is as follows.
\end{definition}

\begin{equation}
iRTR = \sum_{i=1}^n \sum_{i=j}^m rtr_{0\_i,j}
\end{equation}

The $iRTR$ is strictly related to each $irt_{i}$ and the values of $rtr_{i}$ and $rtl_{i}$ are dependent of the $ch$, $vth$ and $vti$.
The optimal value---100\% protection---for $iRTR$ is obtained for $iCTR= 1 + 1 + ... + 1 = n $. 
This happens only when the there is a 1:1 mapping between each $irs$ and $rt$ inside $P$. This corresponds to perfect implemented shadow stack.
Note that as closer the value of $iRTR$ gets to 1 the least the protection level is.

Note that in general as closer the value of $iRTR$ is to $n$ the more precise the applied CFI policy is and as higher 
the value of $iRTR$ is w.r.t. $n$ the less precise the used CFI based policy is. Note that in case the value of $rtr_{0\_i}$ is high
this does not influence the security level of the CFI policy only in case the target set is not pure (contains many illegitimate call target as a result
of an imprecise analysis). As higher the total number of illegitimate targets added in total the lower the security level is. Note that if
the $rtr_{0\_i}$ has high values (basically there are many illegitimate targets in the set) the security level of the policy drops. The intuition is that we allow to much 
$rt$ for each return site.

% \subsubsection{Indirect Control Flow Transfer Damping} 

\subsubsection{Indirect Callsite Damping} 
\label{Indirect Callsite Damping} 
We next define our indirect call site damping ($CSD$) formula which will be used to measure the runtime cost of 
applying a certain protection schema by associating the number of checks needed $ncn_{i}$ to be performed before each $ics_{i}$ 
can be safely executed.

\begin{definition}[\textbf{CSD}]
 Let $ncn_{0\_i,j}$ be a set containing $m$ checks for each $ics_{0\_i}$ than the $CSD$ metric is as follows.
\end{definition}

\begin{equation}
CSD = \sum_{i=1}^n \sum_{j=1}^m ncn_{0\_i,j} * k
\end{equation}

We assume for simplicity reasons that the cost of each check is $k=1$. Note that this value can be customized (changed) if needed.
$ncn_{i,j}$ can be computed by counting the number of individual runtime checks added for each $ics$.
The optimal value of the $CSD$ formula (i.e., lowest runtime overhead) is obtained when the $CSD$ evaluates to $n$ for a given $P$. 
This corresponds to around 0\% runtime overhead if one each check has negligible runtime cost and is basically obtainable when for each $ics_{i}$ exactly 
one runtime check is added. If the number of checks that have to be performed before each $ics_{i}$ is high $\ge 2$ than the value of $CSD$ will get higher.
Thus, the runtime performance will drop as a consequence.

\subsubsection{Indirect Return Damping} 
We next define our indirect return site damping ($RSD$) formula which will be used to measure precisely the runtime cost of 
applying a certain protection schema by associating the number of checks needed $nrn_{i}$ to be performed before each $irs_{i}$ 
can be safely performed.

\begin{definition}[\textbf{RSD}]
 Let $nrn_{0\_i,j}$ be a set containing $m$ checks for each $irs_{0\_i}$ than the $RSD$ metric is as follows.
\end{definition}

\begin{equation} 
RSD = \sum_{i=1}^n \sum_{j=1}^m nrn_{0\_i,j} * k
\end{equation}

We assume for simplicity reasons that the cost of each check is $k=1$.
$nrn_{0\_i,j}$ can be computed by counting the number of individual runtime checks that are added per $irs$.
The optimal value of the $RSD$ formula (i.e., lowest runtime overhead) is obtained when the $RSD$ evaluates to $n$. 
Where $n$ is the total number of $irs$ in $P$.
This corresponds to around approx. 0\% runtime overhead and is basically obtainable when for each $irs_{i}$ has exactly 
one runtime check before it that has to be performed.
If the number of checks that have to be performed before each $irs_{i}$ is higher than 1 the value of $RSD$ will get higher.
Thus, the runtime performance will drop as a consequence. We assume that runtime performance is direct proportional to the number of checks that have to be performed.

% \subsubsection{Indirect COOP Gadget Availability}
% We will now formalize COOP gadget availability. Also not that gadget linkalability is also important but in the COOP attack this is not important since gadgets don't call each 
% other but rather there is a main loop gadget which calls the gadgets one by one. So gadget linkalibility will be not considered herein.

\subsubsection{Forward COOP Gadget Availability}
\label{Forward COOP Gadget Availability}
We next define our forward-edge based $cg$ availability metric which is used to measure quantitatively the availability of $cg$ per $ics$ after applying a protection policy. 
The $fCGA$ can be thought to be dependent of $iCTR$. The $fCGA$ can help to design CFI protection schemes which target $ict$ that have after them 
a $cg$ and thus could be exploited by $A$. In this way runtime overhead can be kept low by avoiding to insert costly checks which are useless for certain 
indirect control flow transfers targets that do not contain any $cg$ and thus useless for $A$.

\begin{definition}[\textbf{fCGA}]
Let $cgp_{j}$ be a set containing only values of 1 indicating the presence of a $cg$ after a $ict_{i}$ and values of 0 indicating the 
absence of a $cg$ after the $ict_{i}$ (inside the corresponding virtual function). 
$ctr_{i}$ set represents the total number of call targets after applying an ideal policy which is the same ideal policy applied for each $ics_{0\_i}$
than the the $fCGA$ metric is as follows.
\end{definition}

\begin{equation}
fCGA = \sum_{i=1}^n \sum_{j=1}^m cgp_{0\_i,j}
\end{equation}

The set $cgp_{j}$ for a particular $ics_{i}$ can be computed by analyzing the contents of each virtual function corresponding to a 
particular $ict_{i}$.
In case there is no $cg$ after each $ctr_{i}$ present in $P$ than $fCGA$ for the given $P$ evaluates to 0.
In case not all $ics$ in the program are not protected by at least one check before it and from this $ics$ the attacker can access
$cgp_{0\_i,j}$ which evaluate to 1 the lower the protection level is.
As higher the number of protected indirect transfers and higher the number of available $cg$ after 
each of these transfers as closer the value of $fCGA$ will be to $iCTR$ else the value will be lower than $iCTR$.
If all $ie$ are protected but after each of them there is no $cg$ than the value of $fCGA$ is 0 and the checks added are useless.
Ideally each control flow transfer check should protect a $ict$ having after it a $cg$ with the least number of checks possible (i.e., 1).

\subsubsection{Backward COOP Gadget Availability}
We next define our backward COOP gadget availability metric as matter of completeness which is used to measure quantitatively
the availability of $cg$ per $irt$ after 
applying a certain protection schema. 
Note that this metric is not directly relevant to COOP since $irs$ are not used in order to chain COOP gadgets; still we define this metric since it is usable
for other types of CRAs which use $irs$ in order to build gadget chains. In the context of this work we assume that this metric is relevant for COOP.
The $rCGA$ is directly dependent to $iRTR$. The $rCGA$ can help to design CFI protection schemes which target $irt$ that contain after the return address
a $cg$ and thus could be exploited by $A$. In this way runtime overhead can be kept low by avoiding to insert costly checks which are useless for certain 
indirect control flow transfers and thus not available to $A$.

\begin{definition}[\textbf{rCGA}]
Let $cgr_{j}$ be a set containing values of 1 indicating the presence of an $cg$ after a $irt_{i}$ and values of 0 indicating the 
absence of a $cg$ after the $irt_{i}$ than $rtr_{i}$ is the total number of return targets after applying a certain policy for one $rt_{i}$
than the $rCGA$ metric is as follows.
\end{definition}

\begin{equation}
rCGA = \sum_{i=1}^n \sum_{j=1}^m cgr_{0\_i,j}
\end{equation}

The number of legitimate return targets for a $irt_{i}$ is one if the caller/callee calling convention is enforced. 
In case there is no $cg$ after each $irt_{i}$ present in $P$ than $rCGA$ for the given $P$ evaluates to 0.
In case not all $irt$ in the program are protected by at least one check before it and from this $irt$ the attacker can access
$cgp_{0\_i,j}$ which evaluate to 1 the lower the protection level is.
As higher the number of protected indirect transfers and higher the number of available $cg$ after 
each of these transfers as closer the value of $fCGA$ will be to $iRTR$ else the value will be lower than $iCTR$.
If all $ie$ are protected but after each of them there is no $cg$ than the value of $fCGA$ is 0 and the checks added are useless.
Ideally each control flow transfer check should protect a $irt$ having after it a $cg$ with the least number of checks possible (i.e., 1).


% \begin{definition}
% \label{this2}
% Cf. to Definition~\autoref{this1} a $ics_{i}$ is allowed to call a certain $ict$ (virtual function) than
% all the returns in that virtual function are allowed to return to the address next to the $ics_{i}$. 
% \end{definition}
% 
% \begin{property}
% Note that in Definition~\autoref{this2} we assume that the call/callee calling convention is respected.
% \end{property}
% 
% \begin{definition}
% \label{this3}
% In order to compute (cf. Definition~\autoref{this2}) all possible legitimate return addresses for a $irt_{i}$ an algorithm should visit all $ics_{i}$ and forward/associate 
% the addresses located at the next instruction address after that particular $ics_{i}$ to each  $irt_{i}$. 
% \end{definition}
% 
% \begin{property}
% Note that (cf. Definition~\autoref{this3}) in this way the forward edge class based inheritance schema will be enforced to return edges.
% \end{property}
% 
% \begin{property}
% Note that (cf. Definition~\autoref{this3}) that the smallest set of $irt$ that can be enforced for a $irs$ is based on the $mvt$ which basically has to
% be enforced to all return edges.
% \end{property}





==> parts/future.tex <==
In this section we briefly address possible future research directions.

\subsection{Measuring Gadgets Usability}
In order to measure gadget usability for a particular attack first two situations have to taken into account. First, 
in case the pplication was not previously hardened with any policy one can decide based on the gadget set for the attack he/she
wants to perform if a sequence of machine instructions can be used during the attack and it is with reasonable effort reachable.
Second, in case the binary was hardened with a protection policy against code reuse attacks things get more complicated since the attacker
not on has to locate the particular types in the application but he has to know how to avoid getting into the previously inserted checks.
On one hand, in case the checks are easy to spot than he can use what ever gadget he/she can get to. On the other hand, 
if the attacker can not determine which protection mechanism was applied to the program he does only know that the gadget 
is available but not usable for the attack. In order to measure gadget usability the ICFI framework can be extended with metrics which take into account 
individually for each gadget if is protected or not and if a gadget belongs to a certain type of attack.

\subsection{Measuring Gadgets Linkability}
The starting point for a gadget linkalibility metric which basically measures how hard or easy is to link gadgets to each other. First the semantics used to link gadgets have to be defined
and next these have to be related to fCGA and rCGA which basically quantify the presence of a COOP gadget inside a virtual function. 
A good approach in this direction was made by Crafted~\cite{crafted} which present a LLVm compiler based which can determine all possible gadget chains inside a given 
program based on an augmented CFG, instruction mapper and a control flow verifier which basically can be used to determine if it is possible to execute a given instruction
sequences identified by the Instruction Mapper without violating the control-flow restrictions of the defense policy.

\subsection{Measuring Attack Success Rate}
Measuring attack success rate is based on gadget (1) usability,(2) linkability, (3) gadget chain and (4) goal policy. In order to measure success rate 
firs a metric should be able to measure if a certain type of gadget is available and next if this gadget is linkable (can be used in a gadget chain).
First, the gadget chain policy is takes the rational of the attacker w.r.t. what he/she wants to achieves and translates it to the needed gadgets that have to be performed.
This can be mapped to a certain gadget chain. Second, the goal of the attacker has to be determined in terms of what he want to achieve by chaining and calling his gadgets one
by one after each other. Third, the sequence of how he can achieve his goal needs to be mapped to all possible gadget chains which can be formed out of the available gadget set.
An attack is in our understanding sucessfull if the last gadget in the gadget chain was reached and if the goal the result matches with the initial goal of the attacker.
In future we want to derive a metric which can asses the success rate of an attack by taking into account (1-4). 

==> parts/related.tex <==
%\textbf{\textit{Defense Assessment Metrics.}}
AIR~\cite{mingwei:sekar}, fAIR~\cite{vtv:tice}, and AIA~\cite{aia} are currently the only available CFI defense assessment metrics which can be used to assess the protection level offered by state-of-the-art CFI defenses w.r.t. forward-edge transfers. 
However, these metrics provide average values which shed limited insight into the real offered protection level and thus can not be used to compare tools against each other.
% but also the backward-edge target set reduction, the runtime damping of each CFI policy as well as the gadget availability set after a program was 
% hardened with a CFI policy.
Burow \textit{et al.} \cite{cfi:survey} propose two new metrics:
(1) qualitative metric, based on the underlying analysis provide by each of the assessed techniques, and 
(2) quantitative metric, the product of the number of equivalence classes (EC) and the inverse of the size of the largest class (LC).

In contrast to the above presented metrics, we provide a CFI defense assessment framework (\sysname) and a new CFI defense assessing metric ($CTR$) that is based on absolute forward-edge reduction set counting, without averaging the results and which provides precise measurements and facilitates comprehensive CFI defense comparison.

% Finally, we note that the existing forward-edge CFI metrics are used mostly without specifying the total number of callsites contained in the 
% hardened program and providing average numbers can induce the reader into error by giving a false sense of security.

% \textbf{\textit{Static Gadget Discovery.}}
% Wollgast \textit{et al.} \cite{multiarchitecture:wollgast} present a static multi-architecture gadget detection tool based on the analysis
% of the intermediate language (IL) of VEX, which is part of the Valgrind \cite{valgrind} programing debugging framework. The tool can find a series of CFI-resistant gadgets. 
% Compared to \sysname, both tools leave the gadget chain building as a manual effort. In contrast, when using \sysname, it is possible to define a specific CFI-defense policy 
% and search for available gadgets 
% while the tool of Wollgast et al. specifies CFI resistant gadgets by defining their boundaries (start and end instructions). These have to conform to some constraints 
% and respect the normal program control flow of the program in order to be considered CFI resistant. These types of gadgets are more thoroughly described
% by Goktas \textit{et al.} \cite{goktas:outofcontrol}, Schuster \textit{et al.} \cite{schuster:rop}.

% RopDefender \cite{ropdefender}, ROPgadget \cite{ROPgadget}, and Ropper \cite{Ropper} are non-academic gadget detection tools for program binaries. 
% These tools are used to search inside program binaries with the goal to find consecutive machine code instructions which are similar to a previously specified set of rules that define a valid gadget. 
% While performing a fast search, these tools however cannot detect defense-aware gadgets, since these tools do not model the defense applied to the program 
% binary. As such, these tools cannot determine which gadgets are usable after a certain defense was applied. 

%\textbf{\textit{Dynamic Attack Construction.}} 
Another closely related work is Newton~\cite{newton}, a runtime binary analysis tool which relies on taint analysis to help significantly simplify the detection of code reuse gadgets defined as callsite and legal calltarget pairs. 
A substantial difference compared to Newton is that \sysname uses program source code, which captures more precise information about the caller-callee pair than binary analysis based approaches.

% At first, quite effectively as demonstrated by the Newton paper, this tool can model part of the byte memory dependencies in a given program.
% Newton is able to model a series of 
% code reuse defenses by not focusing on a specific attack at a time. Finally, Newton
% is able to craft attacks in the face of several arbitrary memory write constraints. 

There are also other attack construction tools. StackDefiler \cite{losing:control:conti}, comprises of a set of stack corruption attacks that leverage runtime object allocation information in order to bypass fine-grained CFI defenses. %Based on the fact that Indirect Function-Call Checks (IFCC) \cite{vtv:tice} (also valid for VTV) spills critical pointers onto the stack the authors show how CRAs can be built even in presence of a fine-grained CFI defense.
Compared to \sysname which is based on control flow bending to legitimate targets, StackDefiler shows an alternative approach for crafting CRAs. %More specifically, Conti \textit{et al.} show that information disclosure poses a severe threat. They also show that shadow stacks which are not protected through memory isolation are an easy target for the attacker.

% %%commented out for space reasons.
Argument Corruptible Indirect Call Site (ACICS) \cite{jujutsu} gadgets are detected during runtime by the ADT tool, in a similar way as Newton's detects gadgets. 
% Note that the ACICS gadgets are more constrained then those of Newton. For example,
% only attacks where the function pointer and arguments are corruptible on the heap or in global memory are taken into consideration.
% As Newton does not impose so many constraints on the gadgets, it can find depending on the analyzed program more sophisticated attacks where the attack elements can be corrupted in many more complex and indirect ways.
Similar to \sysname, the ADT tool is able to craft an attack in the face of IFCC's CFI defense policy by finding pairs of indirect callsites that match to certain functions 
which can be corrupted during runtime. In contrast, \sysname, is not program input dependent as it is not a runtime tool. Therefore, it can find all corruptible 
indirect callsite and function pairs under a certain modeled CFI policy.

Revery \cite{revery} is another dynamic attack crafting tool
which analyzes a vulnerable program and collects runtime information on the crashing path as for example taint attributes of variables. Revery fails
in some cases to generate an attack due to complicated defense mechanisms of which the tool is not aware. Further the tool fails, in some cases, to generate exploits due to dynamic decisions which have to be made during exploitation. \looseness=-1








==> parts/threatmodel.tex <==
We align our threat model with previous work
by considering a powerful and realistic adversary~\cite{newton, mohan:opaque, just:in:time, trap:crane, coop}. 
More specifically, we rely on deployed and complementary mitigation techniques to achieve a comprehensive coverage.
We assume that the attacker/analyst knows which CFI based defense is applied to a deployed program, has access to the source code of his prospective victim application and to the target binary. We assume that the hardened binary was not generated with the same LLVM based compiler. The target binary is not re-randomized in short intervals. For instance, the attacker can extract knowledge
about the environment and apply this knowledge to the attack.
The program which the attacker wants to attack contains an exploitable 
memory corruption (\textit{e.g.,} buffer overflow) that allows the attacker to corrupt memory objects (\textit{e.g.,} inserting fake objects). 
The attacker relies on an automated gadget discovery tool to craft a CRA
with reduced application knowledge. Further, the attacker's goal is to find gadgets and mount a CRA even 
if state-of-the-art CFI \cite{vtv:tice, zhang:vtrust} defenses are deployed. We deliberately only focus on CFI-based defenses
as this defense class is well explored, evaluated and used in practice \cite{clang:cfi}. 
The system on which the vulnerable application is running
ensures that the memory can be either writable or executable (W$\oplus$X), but not both at the same time (\textit{e.g.,} DEP \cite{dep}). 
Address Space Layout Randomization (ASLR) \cite{aslr} is in place. A perfect shadow stack implementation is also deployed, which makes 
the exploit of CFG returning edges impossible. 
The attacker can therefore only jump at the beginning of a function and not inside due to a coarse-grained forward-edge CFI \cite{mingwei:sekar} defense.
The system on which the vulnerable application runs enforces execute-only memory
pages. This essentially means that the CPU can fetch instructions, while normal read and write accesses trigger an access violation (\textit{e.g.,} XOM \cite{norax:xom}).

